FaceTuneGAN: Face Autoencoder for Convolutional Expression Transfer Using Neural Generative Adversarial Networks

In this paper, we present FaceTuneGAN, a new 3D face model representation decomposing and encoding separately facial identity and facial expression. We propose a first adaptation of image-to-image translation networks, that have successfully been used in the 2D domain, to 3D face geometry. Leveraging recently released large face scan databases, a neural network has been trained to decouple factors of variations with a better knowledge of the face, enabling facial expressions transfer and neutralization of expressive faces. Specifically, we design an adversarial architecture adapting the base architecture of FUNIT and using SpiralNet++ for our convolutional and sampling operations. Using two publicly available datasets (FaceScape and CoMA), FaceTuneGAN has a better identity decomposition and face neutralization than state-of-the-art techniques. It also outperforms classical deformation transfer approach by predicting blendshapes closer to ground-truth data and with less of undesired artifacts due to too different facial morphologies between source and target.

==> commands/comments.tex <==
\newcommand\Comm[3]{
    {\color{#1}\textbf{#2:} \small{#3}}
}

\newcommand\QA[1]{
    \Comm{magenta}{QA}{#1}
}
\newcommand\FD[1]{
    \Comm{teal}{FD}{#1}
}
\newcommand\NO[1]{
    \Comm{orange}{NO}{#1}
}
\newcommand\KB[1]{
    \Comm{red}{KB}{#1}
}
\newcommand\FM[1]{
    \Comm{blue}{FM}{#1}
}

\newcommand\TODO[1]{
    \Comm{red}{TODO}{#1}
}

\definecolor{cadded}{rgb}{0.0,0.8,0.0} 
\newcommand{\added}[1]{\textcolor{cadded}{~#1}}
\newcommand{\remove}[1]{\textcolor{red}{\sout{#1}}}
\newcommand{\replace}[2]{\added{#1} \remove{#2}}

==> commands/utils.tex <==
\newcommand\FIG[1]{
    Fig.\ \ref{#1}
}

\newcommand\TAB[1]{
    Table \ref{#1}
}

\newcommand\SECTION[1]{
    Section \ref{#1}
}
